Estimating the Blood Supply Elasticity: Evidence from a Universal Scale Benefit Scheme

I estimate the semi-elasticity of blood donations with respect to a monetary benefit, namely the waiver of user fees when using the National Health Service, in Portugal. Using within-county variation over time in the value of the benefitI estimate both the unconditional elasticity, which captures overall response of the market, and the conditional elasticity, which holds constant the number of blood drives. This amounts to fixing a measure of the cost of donation to the blood donor. I instrument for the number of blood drives, which is endogenous, using a variable based on the number of weekend days and the proportion of blood drives on weekends. A one euro increase in the subsidy leads 1.8% more donations per 10000 inhabitants, conditional on the number of blood drives. The unconditional effect is smaller. The benefit does not attract new donors, instead it fosters repeated donation. Furthermore, the discontinuation of the benefit lead to a predicted decrease in donations of around 18%, on average. However, I show that blood drives have the potential to effectively substitute monetary incentives in solving market imbalances.

==> fsecond.tex <==
\clearpage


	\begin{figure}[!htb]\caption{Distribution of time between first and second donation, in days}\label{fsecond}
	\centering
	\includegraphics[scale=0.45]{kdens_time_second.png} 
		\begin{mfigsource} 
			Author's compilation based on Portuguese Blood and Transplantation Institute data. 
	\end{mfigsource}

	\end{figure}	


==> tab_r_all.tex <==
\clearpage


\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption[Effect of Benefit on Donations per 10,000 Inhabitants - Model Specifications]{Effect of the Benefit on the Number of Blood Donations per 10000 Inhabitants}\label{tab_r_all}
\bigskip

\begin{tabular}{l*{5}{c}}
\toprule
               &\multicolumn{5}{c}{\tbf{Donations per 10000 Inhabitants} }\\
 		 &Level & IHS &\multicolumn{3}{c}{Log ($x$+ Donations)}\\    
		 & & & 0.1 & 0.01 & 0.001 \\  \cline{4-6}        
\tbf{Euro}                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\ 
\midrule

ED Subsidy          &        0.12  &       0.012  &       0.010  &      0.007  &      0.002  \\
                    &     (0.084)  &    (0.007)\dag&    (0.009)  &     (0.013)  &     (0.017)  \\
\midrule
Mean Dep. Variable &   11.77 &   1.78 &       0.58 &    -0.15 &       -0.84 \\
\midrule
Observations        &       12960  &       12960  &       12960  &       12960  &       12960  \\
\(R^{2}\)           &       0.607  &       0.740  &       0.719  &       0.683  &       0.656  \\
\bottomrule
\end{tabular}
	\begin{mfignotes} 
			Regressions include county and calendar month fixed effects. Standard error clustered at county level. Significance levels:  $\dag$ : 10\% \hspace{1em} $\ast$ : 5\% \hspace{1em} $\ast\ast$ : 1\%
			The hyperbolic sine of 1.78 is equal to 2.90 donations per 10,000 inhabitants. IHS stands for inverse hyperbolic sine transformation.  
			0.58 in the log scale corresponds to 1.78 donations per 10,000 inhabitants.
	\end{mfignotes}

\end{table}



==> tab_r_all_count.tex <==
\clearpage


\begin{sidewaystable}[htbp]
\begin{small} \centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption[Effect of Benefit on Blood Donations per 10000 Inhabitants - Count Models]{Effect of the Benefit on the Number of Blood Donations per 10000 Inhabitants}\label{tab_r_all_count}

\bigskip

\begin{tabular}{l*{7}{c}}

\toprule
               &\multicolumn{7}{c}{\tbf{Donations per 10000 Inhabitants} }\\
	& \multicolumn{3}{c}{Pooled Data} & &  \multicolumn{3}{c}{Random Effects} \\
	      &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)} &  &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)} &\multicolumn{1}{c}{(3)}\\
	                 		 &Poisson & Negative Binomial &Probit &  &Poisson & Negative Binomial &Probit\\ \cline{2-4}\cline{6-8}    
\tbf{Main} \\
ED Subsidy            &       0.036  &       0.044  &        0.16  &  &     0.030  &       0.088  &       0.014  \\
                    &     (0.029)  &     (0.033)  &     (0.025)**&   & (0.002)**&    (0.005)**&     (0.010)  \\

\midrule
$\ln \alpha$             &              &              &              &              &              &              \\
Constant            &              &        1.24  &       &       &        0.72  &              &              \\
                    &              &      (0.11)**&              &&      (0.11)**&              &              \\
\midrule
$ \ln r$                &              &              &          &    &              &              &              \\
Constant            &              &              &              &&              &       -0.43  &              \\
                    &              &              &              &         &     &      (0.12)**&              \\
\midrule
$ \ln r$               &              &              &              &  &            &              &              \\
Constant            &              &              &              &       &       &        0.26  &              \\
                    &              &              &              &              &&      (0.15)\dag&              \\
\midrule
$ \ln \sigma^{2}_{u}$      &              &              &              &&              &              &              \\
Constant            &              &              &              &              &&              &        1.53  \\
                    &              &              &              &              &      &        &      (0.61)* \\
 \midrule
Mean of Dep. Variable & 11.77 & 11.77 & 0.70 & & 11.77 & 11.77 & 0.70 \\
\midrule
Observations        &       12960  &       12960  &       12960  & &      12960  &       12960  &       12960  \\
		
\bottomrule
\end{tabular}
	\begin{mfignotes} 
			Standard error clustered at county level. Significance levels:  $\dag$ : 10\% \hspace{1em} $\ast$ : 5\% \hspace{1em} $\ast\ast$ : 1\%
			IHS stands for inverse hyperbolic sine transformation. 
	\end{mfignotes}
\end{small}
\end{sidewaystable}



==> tab_r_all_tpm.tex <==
\clearpage


\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption[Effect of Benefit on Donations per 10,000 Inhabitants - Two Part Model]{Effect of the Benefit on the Number of Blood Donations per 10000 Inhabitants}\label{tab_r_all_tpm}
\bigskip

\begin{tabular}{l*{3}{c}}
\toprule
               &\multicolumn{2}{c}{\tbf{Donations per 10000 Inhabitants} }\\

                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)} \\
                    &\multicolumn{1}{c}{OLS}&\multicolumn{1}{c}{GLM} \\ 
\midrule
\tbf{Probit}              &              &                         \\
ED Subsidy          &     -0.002  &     -0.002   \\
                    &     (0.014)  &     (0.014)   \\
\midrule
\tbf{Donations $>0$}              &              &                         \\
ED Subsidy          &       0.044  &   0.017        \\
                    &      (0.11)  &    (0.012)                \\

\midrule
Mean Dep. Variable &   \multicolumn{2}{c}{11.77}  \\
\midrule
Observations        &        8400  &        8400   \\
Log Likelihood                  &    -43035  &    -32382  \\
AIC                 &     86415  &     65109    \\
BIC                 &     87625  &     66319   \\

\bottomrule
\end{tabular}
	\begin{mfignotes} 
			Regressions include county and calendar month fixed effects. Standard error clustered at county level. Significance levels:  $\dag$ : 10\% \hspace{1em} $\ast$ : 5\% \hspace{1em} $\ast\ast$ : 1\%
			GLM: Generalized linear model, with gamma family distribution and log link. 
	\end{mfignotes}

\end{table}



==> tab_r_sstage.tex <==
\clearpage


\begin{sidewaystable}[htbp]
\begin{small} \centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption[Effect of Benefit on Blood Donations per 10000 Inhabitants - Two Stage Least Squares - Model Specifications]{Effect of the Benefit on the Number of Blood Donations per 10000 Inhabitants}\label{tab_r_sstage}

\bigskip

\begin{tabular}{l*{10}{c}}

\toprule
               &\multicolumn{10}{c}{\tbf{Donations per 10000 Inhabitants} }\\
 		 &Level & IHS &\multicolumn{3}{c}{Log ($x$+ Donations)} &  &IHS &\multicolumn{3}{c}{Log ($x$+ Donations)}\\    
		 & & & 0.1 & 0.01 & 0.001 & & & 0.1 & 0.01 & 0.001 \\  \cline{4-6} \cline{9-11}        
	                &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)} &\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)} & &\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)} &\multicolumn{1}{c}{(5)}\\
\midrule
ED Subsidy          &        0.39  &       0.028  &       0.027  &       0.025  &       0.022  &   &    0.018  &      0.0034  &     -0.0051  &      -0.010  \\
                    &      (0.19)* &     (0.011)* &     (0.014)\dag&     (0.018)  &     (0.022)  &   & (0.0084)* &    (0.0086)  &     (0.012)  &     (0.017)  \\
Blood Drives             &        41.8  &        2.41  &        2.60  &        2.85  &        3.07  &              &              &              &              \\
                    &      (4.73)**&      (0.21)**&      (0.23)**&      (0.27)**&      (0.30)**&              &              &              &              \\

IHS Blood Drives   &              &              &       &       &              &              &        2.85  &              &              &              \\
                    &              &              &              &   &           &              &      (0.22)**&              &              &              \\
Ln(0.1+ Drives)   &              &              &              &&              &              &              &        1.03  &              &              \\
                    &              &              &              &        &      &              &              &     (0.072)**&              &              \\
Ln(0.01+ Drives) &              &              &              &   &           &              &              &              &        0.55  &              \\
                    &              &              &              &             & &              &              &              &     (0.043)**&              \\
Ln(0.001+ Drives)  &              &              &              &     &         &              &              &              &              &        0.38  \\
                    &              &              &              &              &  &            &              &              &              &     (0.033)**\\


 \midrule
Mean of Dep. Variable & 11.77 & 1.79 & 0.58 & -0.15 & -0.85 & &  1.79 & 0.58 & -0.15 & -0.85 \\
Weak Identification F-stat      &      135.7  & 135.7 & 135.7 & 135.7 & 135.7 &     &     207.4  &       590.2  &       863.8  &       901.9  \\
      \medskip 
Observations        &       12960  &       12960  &       12960  &       12960  &       12960  & &       12960  &       12960  &       12960  &       12960  \\
\(R^{2}\)           &       0.152  &       0.049  &       0.036  &       0.026  &       0.020  &    &   0.248  &       0.223  &       0.126  &       0.079  \\
		
\bottomrule
\end{tabular}
	\begin{mfignotes} 
			Regressions include county and calendar month fixed effects. Standard error clustered at county level. Significance levels:  $\dag$ : 10\% \hspace{1em} $\ast$ : 5\% \hspace{1em} $\ast\ast$ : 1\%
			IHS stands for inverse hyperbolic sine transformation. Blood Drives per 10,000 inhabitants.
			The instrumental variable {\em IV:Weekend} measures the number of weekend or holiday days, in a given county/month, multiplied by a county's overall weekend blood drive rate. 
			This rate is computed as the proportion of blood drives held in a weekend, as opposed to weekday, for that county. 
	\end{mfignotes}
\end{small}
\end{sidewaystable}



==> tab_sstage_cat.tex <==
\clearpage


\begin{sidewaystable}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption[Effect of Benefit on Blood Donations per 10000 Inhabitants - Two Stage Least Squares]{Effect of the Benefit on the Number of Blood Donations per 10000 Inhabitants}\label{tab_sstage}

\bigskip

\begin{tabular}{l*{9}{c}}

	&\multicolumn{9}{c}{Two Stage Least Squares}\\   
\toprule
               &\multicolumn{4}{c}{\tbf{Donations per 10000 Inhabitants}} &  &\multicolumn{4}{c}{\tbf{IHS Donations per 10000 Inhabitants}} \\
              & \multicolumn{4}{c}{Mean=11.77}  & & \multicolumn{4}{c}{Mean=1.78} \\
	                &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)} &\multicolumn{1}{c}{(4)}& &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)} &\multicolumn{1}{c}{(4)}\\
	                &\multicolumn{1}{c}{OLS}&\multicolumn{1}{c}{OLS}&\multicolumn{1}{c}{2SLS} &\multicolumn{1}{c}{2SLS}& &\multicolumn{1}{c}{OLS}&\multicolumn{1}{c}{OLS}&\multicolumn{1}{c}{2SLS} &\multicolumn{1}{c}{2SLS}\\
	                & & &\multicolumn{1}{c}{IV level} &\multicolumn{1}{c}{IV IHS}& & & &\multicolumn{1}{c}{IV level} &\multicolumn{1}{c}{IV IHS}\\ \cline{2-5} \cline{7-10}

ED Subsidy          &        0.12  &        0.28  &        0.39  &        0.36  &    &   0.012  &       0.016  &       0.018  &       0.018  \\
                    &     (0.084)  &      (0.10)**&      (0.19)* &      (0.17)* &  &  (0.007)\dag&    (0.006)* &    (0.008)* &    (0.008)* \\
Blood Drives          &              &        24.8  &        41.8  &        38.2  &              &              &              &              \\
                    &              &      (5.31)**&      (4.73)**&      (4.66)**&              &              &              &              \\
IHS Blood Drives   &              &              &              &              &          &    &        1.91  &        2.85  &        2.75  \\
                    &              &              &              &              &              &    &  (0.19)**&      (0.22)**&      (0.22)**\\
 \midrule
Weak Identification F-stat       &              &              &       135.7  &       138.0  &      &        &              &       207.4  &       207.5  \\
                    \midrule 
Observations       &       12960  &       12960  &       12960  &       12960  &  &     12960  &       12960  &       12960  &       12960  \\
\(R^{2}\)           &       0.607  &       0.720  &       0.152  &       0.202  &    &   0.740  &       0.825  &       0.248  &       0.262  \\
\bottomrule
\end{tabular}
	\begin{mfignotes} 
			Regressions include county and calendar month fixed effects. Standard error clustered at county level. Significance levels:  $\dag$ : 10\% \hspace{1em} $\ast$ : 5\% \hspace{1em} $\ast\ast$ : 1\%
			IHS stands for inverse hyperbolic sine transformation. Blood Drives per 10,000 inhabitants.
			The instrumental variable {\em IV:Weekend} measures the number of weekend or holiday days, in a given county/month, multiplied by a county's overall weekend blood drive rate. 
			This rate is computed as the proportion of blood drives held in a weekend, as opposed to weekday, for that county. 
	\end{mfignotes}
\end{sidewaystable}


